GIQ: Benchmarking 3D Geometric Reasoning of Vision Foundation Models with Simulated and Real Polyhedra

Modern monocular 3D reconstruction methods and vision-language models (VLMs) demonstrate impressive results on standard benchmarks, yet recent works cast doubt on their true understanding of geometric properties. We introduce GOQ, a comprehensive benchmark specifically designed to evaluate the geometric reasoning capabilities of vision and vision-language foundation models. GIQ comprises synthetic and real-world images and corresponding 3D meshes of diverse polyhedra covering varying levels of complexity and symmetry, from Platonic, Archimedean, Johnson, and Catalan solids to stellations and compound shapes. Through systematic experiments involving monocular 3D reconstruction, 3D symmetry detection, mental rotation tests, and zero-shot shape classification tasks, we reveal significant shortcomings in current models. State-of-the-art reconstruction algorithms trained on extensive 3D datasets struggle to reconstruct even basic geometric Platonic solids accurately. Next, although foundation models may be shown via linear and non-linear probing to capture specific 3D symmetry elements, they falter significantly in tasks requiring detailed geometric differentiation, such as mental rotation. Moreover, advanced vision-language assistants such as ChatGPT, Gemini and Claud exhibit remarkably low accuracy in interpreting basic shape properties such as face geometry, convexity, and compound structures of complex polyhedra. GIQ is publicly available at toomanymatts.github.io/giq-benchmark/, providing a structured platform to benchmark critical gaps in geometric intelligence and facilitate future progress in robust, geometry-aware representation learning.

==> table_mrt_probe.tex <==
% \begin{table}[t]
%   \centering
%   \renewcommand{\arraystretch}{1.1}
%   \newcommand{\hdrstack}[1]{%
%   \shortstack[c]{\rule{0pt}{1.1\normalbaselineskip}#1}}

%   \begin{tabular}{|
%       >{\centering\arraybackslash}m{2cm}
%     | ccc
%     | ccc
%     | ccc
%     |}
%     \hline
%     \noalign{\vskip 0pt}% not strictly needed now
%     \multirow[c]{-1.5}{*}{\textbf{Featurizer}} &
%       \multicolumn{3}{c|}{\hdrstack{Train\\(syn,syn)\,$\to$\,Test\\(syn,syn)}} &
%       \multicolumn{3}{c|}{\hdrstack{Train\\(syn,syn)\,$\to$\,Test\\(syn,wild)}} &
%       \multicolumn{3}{c|}{\hdrstack{Train\\(syn,wild)\,$\to$\,Test\\(syn,wild)}} \\
%     \cline{2-10}
%       & Pos & Neg & Avg & Pos & Neg & Avg & Pos & Neg & Avg \\
%     \hline
%     CLIP~\cite{radford2021learning}       & 0.97 & 0.48 & 0.64 & 0.36 & 0.51 & 0.44 & 0.72 & 0.39 & 0.55 \\
%     ConvNext~\cite{liu2022convnet}   & 0.99 & 0.54 & 0.70 & 0.43 & 0.51 & 0.47 & 0.69 & 0.60 & 0.65 \\
%     deit\_iii~\cite{touvron2022deit}  & 0.90 & 0.59 & 0.70 & 0.35 & 0.61 & 0.48 & 0.72 & 0.41 & 0.56 \\
%     DINO~\cite{caron2021emerging}       & 0.95 & 0.64 & 0.74 & 0.36 & 0.51 & 0.44 & 0.62 & 0.54 & 0.58 \\
%     DINOv2~\cite{oquab2023dinov2}      & 0.94 & 0.71 & 0.79 & 0.36 & 0.52 & 0.44 & 0.77 & 0.43 & 0.60 \\
%     DreamSim~\cite{fu2023dreamsim}   & 0.99 & 0.65 & 0.77 & 0.36 & 0.51 & 0.44 & 0.74 & 0.49 & 0.62 \\
%     MAE~\cite{he2022masked}        & 0.99 & 0.64 & 0.76 & 0.36 & 0.51 & 0.44 & 0.75 & 0.42 & 0.58 \\
%     SAM~\cite{foret2020sharpness}        & 0.94 & 0.68 & 0.77 & 0.36 & 0.52 & 0.44 & 0.73 & 0.42 & 0.57 \\
%     SigLip~\cite{zhai2023sigmoid}     & 0.94 & 0.67 & 0.76 & 0.36 & 0.51 & 0.44 & 0.74 & 0.54 & 0.64 \\
%     \hline
%   \end{tabular}
%   \caption{Classification accuracy (\%) on the Mental Rotation Test (MRT) across three settings: synthetic-to-synthetic, synthetic-to-mixed (synthetic+wild), and mixed-to-mixed. For each setting, “Pos” and “Neg” report accuracy on same-object (rotated) and different-object pairs, respectively, and “Avg” is their weighted mean. \mm{remove avg, maybe barplot with horizontal line for chance, maybe remove pos too. maybe both-both and rest is in sup.} }
%   \label{tab:mrt_featurizers}
% \end{table}









% \begin{table}[]
%   \centering
%   % reduce horizontal padding slightly
%   \setlength{\tabcolsep}{4pt}
%   \begin{tabular}{|
%       >{\centering\arraybackslash}p{3cm}|
%       >{\centering\arraybackslash}p{3cm}|
%       >{\centering\arraybackslash}p{3cm}|
%       >{\centering\arraybackslash}p{3cm}|
%     }
%     \hline
%     \multirow{2}{*}{Featurizer} &
%       \multicolumn{3}{c|}{MRT Accuracy on \textit{hard} test set} \\ 
%     \cline{2-4}
%       & Train (syn,syn)\(\to\)Test (syn,syn) 
%       & Train (syn,syn)\(\to\)Test (syn,wild) 
%       & Train (syn,wild)\(\to\)Test (syn,wild) \\ 
%       \hline

%     CLIP       & 0.64 & 0.44 & 0.55 \\
%     ConvNext   & 0.70 & 0.47 & 0.65 \\
%     deit\_iii  & 0.70 & 0.48 & 0.56 \\
%     DINO       & 0.74 & 0.44 & 0.58 \\
%     DINOv2     & 0.79 & 0.44 & 0.60 \\
%     DreamSim   & 0.77 & 0.44 & 0.62 \\
%     MAE        & 0.76 & 0.44 & 0.58 \\
%     SAM        & 0.77 & 0.44 & 0.57 \\
%     SigLip     & 0.76 & 0.44 & 0.64 \\
%     \hline

%   \end{tabular}
%   \caption{Accuracy on the Mental Rotation Test (MRT) task using the absolute feature difference \(|e_1 - e_2|\). “Train (X)\(\to\)Test (Y)” denotes the training and testing domains. All results are reported on the \textit{hard} test set, where only pairs of similar shapes are evaluated. Results for raw subtraction \((e_1 - e_2)\) and feature concatenation \(\mathrm{concat}(e_1, e_2)\) are in the supplementary; \(|e_1 - e_2|\) performed best. \mm{report TP TN} \mm{center featurizer }}

%   \label{tab:mrt_featurizers}
% \end{table}


    % \multirow{2}{*}{ } &
    %   \multicolumn{3}{c|}{$|e_1 - e_2|$} \\ \hline
    % --- Subtraction ---
    % \multirow{2}{*}{ } &
    %   \multicolumn{3}{c|}{($e_1 - e_2$)} \\ 
    % \hline
    % CLIP       & 0.36 & 0.39 & 0.56 \\
    % ConvNext   & 0.51 & 0.49 & 0.54 \\
    % deit\_iii  & 0.45 & 0.46 & 0.53 \\
    % DINO       & 0.48 & 0.49 & 0.49 \\
    % DINOv2     & 0.53 & 0.51 & 0.45 \\
    % DreamSim   & 0.38 & 0.34 & 0.55 \\
    % MAE        & 0.37 & 0.34 & 0.53 \\
    % SAM        & 0.47 & 0.48 & 0.50 \\
    % SigLip     & 0.50 & 0.44 & 0.54 \\
    % \hline
    % \multirow{2}{*}{ } &
    %   \multicolumn{3}{c|}{concat($e_1, e_2$)} \\ 
    % \hline
    % CLIP       & 0.35 & 0.56 & 0.58 \\
    % ConvNext   & 0.46 & 0.50 & 0.52 \\
    % deit\_iii  & 0.41 & 0.54 & 0.54 \\
    % DINO       & 0.52 & 0.52 & 0.54 \\
    % DINOv2     & 0.57 & 0.48 & 0.60 \\
    % DreamSim   & 0.38 & 0.55 & 0.55 \\
    % MAE        & 0.41 & 0.52 & 0.53 \\
    % SAM        & 0.37 & 0.56 & 0.59 \\
    % SigLip     & 0.36 & 0.44 & 0.54 \\
    % \hline

    % \begin{table}[h!]
%   \centering
%   \setlength{\tabcolsep}{2pt}
%   \renewcommand{\arraystretch}{1.3}
%   \begin{tabular}{|c|ccc|ccc|ccc|}
%     \hline
%     \multirow{3}{*}{\textbf{Featurizer}} & \multicolumn{9}{c|}{\textbf{MRT Accuracy on \textit{hard} test set}} \\ 
%     \cline{2-10}
%      & \multicolumn{3}{c|}{Train (syn,syn)$\to$Test (syn,syn)} 
%      & \multicolumn{3}{c|}{Train (syn,syn)$\to$Test (syn,wild)} 
%      & \multicolumn{3}{c|}{Train (syn,wild)$\to$Test (syn,wild)} \\ 
%     \cline{2-10}
%     & Pos & Neg & Avg & Pos & Neg & Avg & Pos & Neg & Avg \\
%     \hline
%     CLIP       & - & - & 0.64 & - & - & 0.44 & - & - & 0.55 \\
%     ConvNext   & - & - & 0.70 & - & - & 0.47 & - & - & 0.65 \\
%     deit\_iii  & - & - & 0.70 & - & - & 0.48 & - & - & 0.56 \\
%     DINO       & - & - & 0.74 & - & - & 0.44 & - & - & 0.58 \\
%     DINOv2     & - & - & 0.79 & - & - & 0.44 & - & - & 0.60 \\
%     DreamSim   & - & - & 0.77 & - & - & 0.44 & - & - & 0.62 \\
%     MAE        & - & - & 0.76 & - & - & 0.44 & - & - & 0.58 \\
%     SAM        & - & - & 0.77 & - & - & 0.44 & - & - & 0.57 \\
%     SigLip     & - & - & 0.76 & - & - & 0.44 & - & - & 0.64 \\
%     \hline
%   \end{tabular}
%   \caption{Accuracy on the Mental Rotation Test (MRT) task using the absolute feature difference $|e_1 - e_2|$. “Train (X)$\to$Test (Y)” denotes training and testing domains. Each domain combination is reported separately for positive pairs (Pos), negative pairs (Neg), and average accuracy (Avg). All results are reported on the \textit{hard} test set, containing pairs of visually similar shapes. Results for raw subtraction $(e_1 - e_2)$ and concatenation $\mathrm{concat}(e_1, e_2)$ are in the supplementary material; absolute difference $|e_1 - e_2|$ performed best.}
%   \label{tab:mrt_featurizers}
% \end{table}
